Self-selection of Information and Belief Update: An Experiment on COVID-19 Vaccine Information Acquisition

How does the endogenous selection of information shape belief formation? In observational settings, individuals only consume information they choose, making it impossible to observe how they would respond to information they actively avoid. We address this identification challenge using a randomized experiment on COVID-19 vaccines in Taiwan. After eliciting subjects' preferences over vaccine-specific reports, we randomly assign them to receive either their chosen or unchosen information, orthogonalizing selection from exposure. We find subjects are more likely to select information about vaccines they already perceive as more effective. Conditional on receiving information, belief updating is substantially larger when the information was self-selected, even after controlling for prior-posterior disagreement. These findings highlight endogenous information demand as a central determinant of persuasion, suggesting that increasing information availability alone may be insufficient when individuals rationally filter out options they perceive as less relevant to their decision-making.

==> learning_group.tex <==
\begin{tabular}{l*{4}c}\hline\hline
&
\multicolumn{4}{c}{\emph{Learning:}
$|$
PreError
$|-|$
PostError
$|$}\\
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
                    &    Efficacy         &Hospitalization         &    Efficacy         &Hospitalization         \\
\hline
                    &                     &                     &                     &                     \\
$|$ Pre-treatment Error $|$&                     &                     &       0.336\sym{***}&       0.422\sym{***}\\
                    &                     &                     &    (0.0257)         &    (0.0323)         \\
\emph{Information Demand}&                     &                     &                     &                     \\
Selected Top 3 -- Received&       4.410\sym{***}&       5.530\sym{***}&       8.086\sym{***}&       12.98\sym{***}\\
                    &     (0.649)         &     (0.823)         &     (0.641)         &     (0.959)         \\
\hfill -- Not Received&       3.053\sym{***}&       4.972\sym{***}&       6.595\sym{***}&       10.72\sym{***}\\
                    &     (0.859)         &     (1.470)         &     (0.784)         &     (1.308)         \\
Not Selected Top 3 -- Received&       2.474\sym{*}  &       3.395\sym{*}  &       5.724\sym{***}&       9.249\sym{***}\\
                    &     (1.169)         &     (1.700)         &     (1.117)         &     (1.671)         \\
\hfill -- Not Received&       1.327         &       3.826\sym{*}  &       3.736\sym{**} &       7.652\sym{***}\\
                    &     (1.311)         &     (1.849)         &     (1.156)         &     (1.662)         \\
Not Top 3 -- Received&       4.500\sym{***}&       6.337\sym{***}&       5.220\sym{***}&       7.452\sym{***}\\
                    &     (1.055)         &     (1.504)         &     (0.971)         &     (1.401)         \\
\hfill -- Not Received&           0         &           0         &           0         &           0         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         \\
Constants           &       0.732         &      -2.405         &      -8.952\sym{***}&      -19.15\sym{***}\\
                    &     (1.861)         &     (3.285)         &     (1.417)         &     (2.818)         \\
\hline
Treatment Effects in \dots&                     &                     &                     &                     \\
Selected Top 3      &       1.357         &       0.558         &       1.491\sym{*}  &       2.256\sym{*}  \\
                    &     (0.750)         &     (1.336)         &     (0.655)         &     (1.057)         \\
Not Selected Top 3  &       1.147         &      -0.431         &       1.987         &       1.597         \\
                    &     (1.544)         &     (2.125)         &     (1.333)         &     (1.859)         \\
Not Top 3           &       4.500\sym{***}&       6.337\sym{***}&       5.220\sym{***}&       7.452\sym{***}\\
                    &     (1.055)         &     (1.504)         &     (0.971)         &     (1.401)         \\
\hline
Observations        &        3160         &        3160         &        3160         &        3160         \\
Subjects            &         632         &         632         &         632         &         632         \\
 \hline\hline \multicolumn{5}{l}{Standard errors in parentheses.  Family income, college majors, and sex are controlled.} \\                 \multicolumn{5}{l}{\sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)} \end{tabular}


==> learning_group_belowmed.tex <==
\begin{tabular}{l*{4}c}\hline\hline
&
\multicolumn{4}{c}{\emph{Learning:}
$|$
PreError
$|-|$
PostError
$|$}\\
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
                    &    Efficacy         &Hospitalization         &    Efficacy         &Hospitalization         \\
\hline
                    &                     &                     &                     &                     \\
$|$ Pre-treatment Error $|$&                     &                     &       0.588\sym{***}&       0.630\sym{***}\\
                    &                     &                     &    (0.0633)         &    (0.0690)         \\
\emph{Information Demand}&                     &                     &                     &                     \\
Selected Top 3 -- Received&       4.293\sym{***}&       4.595\sym{***}&       4.524\sym{***}&       5.358\sym{***}\\
                    &     (0.650)         &     (1.053)         &     (0.625)         &     (1.055)         \\
\hfill -- Not Received&       2.560\sym{**} &       2.268         &       2.852\sym{***}&       2.916\sym{*}  \\
                    &     (0.871)         &     (1.311)         &     (0.822)         &     (1.299)         \\
Not Selected Top 3 -- Received&       1.772         &       3.035\sym{*}  &       2.145\sym{*}  &       3.274\sym{*}  \\
                    &     (1.126)         &     (1.522)         &     (1.085)         &     (1.506)         \\
\hfill -- Not Received&       0.303         &       2.385         &       0.884         &       2.105         \\
                    &     (1.198)         &     (1.717)         &     (1.172)         &     (1.697)         \\
Not Top 3 -- Received&       0.643         &       1.631         &       0.677         &       1.696         \\
                    &     (1.135)         &     (1.835)         &     (1.115)         &     (1.817)         \\
\hfill -- Not Received&           0         &           0         &           0         &           0         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         \\
Constants           &      -5.117\sym{***}&      -11.03\sym{**} &      -9.345\sym{***}&      -16.77\sym{***}\\
                    &     (1.113)         &     (3.505)         &     (1.238)         &     (3.656)         \\
\hline
Treatment Effects in \dots&                     &                     &                     &                     \\
Selected Top 3      &       1.733\sym{*}  &       2.326\sym{*}  &       1.672\sym{*}  &       2.442\sym{*}  \\
                    &     (0.716)         &     (1.139)         &     (0.666)         &     (1.118)         \\
Not Selected Top 3  &       1.469         &       0.650         &       1.261         &       1.169         \\
                    &     (1.334)         &     (1.584)         &     (1.284)         &     (1.599)         \\
Not Top 3           &       0.643         &       1.631         &       0.677         &       1.696         \\
                    &     (1.135)         &     (1.835)         &     (1.115)         &     (1.817)         \\
\hline
Observations        &        1601         &        1591         &        1601         &        1591         \\
Subjects            &         577         &         522         &         577         &         522         \\
 \hline\hline \multicolumn{5}{l}{Standard errors in parentheses.  Family income, college majors, and sex are controlled.} \\                 \multicolumn{5}{l}{\sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)} \end{tabular}


==> learning_treatment.tex <==
\begin{tabular}{l*{4}c}\hline\hline
&
\multicolumn{4}{c}{\emph{Learning:}$|$
PreError
$|-|$
PostError
$|$}\\
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
                    &    Efficacy         &Hospitalization         &Adverse Events         &   Severe AE         \\
\hline
$|$ Pre-treatment Error $|$&       0.290\sym{***}&       0.353\sym{***}&       0.553\sym{***}&       0.310\sym{***}\\
                    &    (0.0247)         &    (0.0315)         &    (0.0267)         &    (0.0295)         \\
Top 3               &      -0.356         &       0.701         &       1.008         &       1.655         \\
                    &     (0.797)         &     (1.306)         &     (0.714)         &     (1.878)         \\
Assigned            &       0.423         &       1.011         &       0.533         &       2.089         \\
                    &     (0.731)         &     (1.367)         &     (0.717)         &     (1.889)         \\
Constants           &      -3.352\sym{*}  &      -10.13\sym{***}&      -17.40\sym{***}&      -11.65\sym{**} \\
                    &     (1.400)         &     (2.716)         &     (1.423)         &     (3.785)         \\
\hline
Observations        &        3160         &        3160         &        3160         &        3160         \\
Subjects            &         632         &         632         &         632         &         632         \\
{hline 108}
Standard errors in parentheses.


==> obsolete_theory.tex <==
\subsection{Proof of Proposition 1}
We first show the comparative statics of $D(\cdot)$ in $\overline{v}-x$.
First consider the case that $\overline{v} \geq x$. 
Thus
$$D(\overline{v}-x,\gamma,c)= v_1 -v_0-c = v_1-\overline{v}  -c.$$
Note that
\begin{align}
v_1-\overline{v} 
=& \int \mathbb{E}_s[v(s)|\varepsilon] \dd \Phi\left(\varepsilon\right)-\overline{v} \nonumber \\
=&(\overline{v}-x)\int \Phi\left(z^*\right) \dd \Phi\left(\varepsilon\right)
-(\overline{v}-x) \label{eq:D1}\\
&+ \int \frac{\sigt\varepsilon}{1+\gamma}\left(1-\Phi\left(z^*\right)\right) \dd \Phi\left(\varepsilon\right) \label{eq:D2}\\
&- \int\left(\frac{\sigs}{1+\gamma}\right)\phi\left(z^*\right) \dd \Phi\left(\varepsilon\right), \label{eq:D3}
\end{align}
where $z^* = \frac{(1+\gamma)(\overline{v}-x)-\sigt \varepsilon}{\sigs}$, 
and $\varepsilon\sim N(0,1)$.
Taking partial derivative of (\ref{eq:D1}) with respect to $\overline{v}-x$, we can find
\begin{align}
&\int \Phi\left(z^*\right) \dd \Phi\left(\varepsilon\right)
+(\overline{v}-x)\int \left(\frac{1+\gamma}{\sigs}\right)\phi\left(z^*\right) \dd \Phi\left(\varepsilon\right) -1\nonumber\\
=&\Phi\left(\frac{(1+\gamma)(\overline{v}-x)}{\sqrt{\sigt+\sigs}}\right)
+(\overline{v}-x)\int \left(\frac{1+\gamma}{\sigs}\right)\phi\left(z^*\right) \dd \Phi\left(\varepsilon\right) -1.\label{eq:D1d}
\end{align}
We can rewrite (\ref{eq:D2}) as
\begin{align}
\frac{\sigt}{1+\gamma}\int \varepsilon \dd \Phi\left(\varepsilon\right)
-\int \frac{\sigt\varepsilon}{1+\gamma}\Phi\left(z^*\right)\dd \Phi\left(\varepsilon\right)
=-\int \frac{\sigt\varepsilon}{1+\gamma}\Phi\left(z^*\right)\dd \Phi\left(\varepsilon\right).
\label{eq:D2a}
\end{align}
Taking partial derivative of (\ref{eq:D2a}) with respect to $\overline{v}-x$, we can find
\begin{align}
&-\int \frac{\sigt\varepsilon}{1+\gamma}\cdot\frac{1+\gamma}{\sigs}\phi\left(z^*\right)\dd \Phi\left(\varepsilon\right)\nonumber\\
=&-\int \frac{\sigt\varepsilon}{\sigs}\phi\left(z^*\right)\dd \Phi\left(\varepsilon\right).\label{eq:D2d}
\end{align}
Taking partial derivative of (\ref{eq:D3}) with respect to $\overline{v}-x$, we can find
\begin{align}
&- \int\left(\frac{\sigs}{1+\gamma}\right)\left(\frac{1+\gamma}{\sigs}\right)\left(-z^*\right)\phi\left(z^*\right) \dd \Phi\left(\varepsilon\right) \nonumber\\
=&  \int\frac{(1+\gamma)(\overline{v}-x)-\sigt \varepsilon}{\sigs}\phi\left(z^*\right) \dd \Phi\left(\varepsilon\right) \nonumber\\
=& (\overline{v}-x)\int\frac{1+\gamma}{\sigs}\phi\left(z^*\right) \dd \Phi
- \int\frac{\sigt\varepsilon}{\sigs}\phi\left(z^*\right) \dd \Phi
\left(\varepsilon\right).\label{eq:D3d}
\end{align}
Combining (\ref{eq:D1d}), (\ref{eq:D2d}), and (\ref{eq:D3d}),
we can find the partial derivative of $v_1-\overline{v}-c$ with respect to $\overline{v}-x$ is
\begin{align}
\Phi\left(\frac{(1+\gamma)(\overline{v}-x)}{\sqrt{\sigt+\sigs}}\right)-1 \leq 0.
\end{align}
Hence $D(\cdot)$ is decreasing in $\overline{v}-x$ when $\overline{v}\geq x$.

The derivation of the partial derivative when $\overline{v}<x$ is similar, where the partial derivative is
\begin{align}
\Phi\left(\frac{(1+\gamma)(\overline{v}-x)}{\sqrt{\sigt+\sigs}}\right) \geq 0.
\end{align}
Hence $D(\cdot)$ is increasing in $\overline{v}-x$ when $\overline{v}< x$.

Then we show the comparative statics of $D(\cdot)$ in $\sigma_\theta$.
Denote
$${\gamma'}_\theta= \frac{\partial \gamma}{\partial \sigma_\theta} 
= \frac{-2\gamma}{\sigma_\theta}$$
and 
$${z'}_\theta= \frac{\partial z^*}{\partial \sigma_\theta} 
= \frac{(\overline{v}-x){\gamma'}_\theta - \varepsilon}{\sigma_s}.$$
Taking partial derivative of (\ref{eq:D1}) with respect to $\sigma_\theta$, we can find
$$(\overline{v}-x)\int {z'}_\theta \phi\left(z^*\right) \dd \Phi(\varepsilon).$$
Taking partial derivative of (\ref{eq:D2a}) with respect to $\sigma_\theta$, we can find
\begin{align*}
&-\int\frac{\varepsilon(1+\gamma)-\sigma_\theta\varepsilon{\gamma'}_\theta}{(1+\gamma)^2}\Phi\left(z^*\right)
+\frac{\sigma_\theta\varepsilon}{1+\gamma}{z'}_\theta \phi\left(z^*\right) \dd \Phi(\varepsilon)\\
=&-\int\frac{\varepsilon(1+3\gamma)}{(1+\gamma)^2}\Phi\left(z^*\right)
+\frac{\sigma_\theta\varepsilon}{1+\gamma}{z'}_\theta \phi\left(z^*\right) \dd \Phi(\varepsilon)
\end{align*}
Taking partial derivative of (\ref{eq:D3}) with respect to $\sigma_\theta$, we can find
$$-\int \frac{\sigs}{(1+\gamma)^2}{\gamma'}_\theta\phi\left(z^*\right) 
+ \frac{\sigs}{1+\gamma}{z'}_\theta (-z^*)\phi\left(z^*\right) \dd \Phi(\varepsilon).$$
Summing up, the partial derivative becomes
\begin{align}
\frac{1+3\gamma}{(1+\gamma)^2}\int -\varepsilon\Phi\left(z^*\right)\dd \Phi(\varepsilon)
-\int \frac{\sigs}{(1+\gamma)^2}{\gamma'}_\theta\phi\left(z^*\right) \dd \Phi(\varepsilon),\label{eq:Dt1}
\end{align}
where 
\begin{align*}
\int -\varepsilon\Phi\left(z^*\right)\dd \Phi(\varepsilon)
=& \int -\varepsilon\phi(\varepsilon)\Phi\left(z^*\right)\dd\varepsilon\\
=&\phi(\varepsilon)\Phi\left(z^*\right)\bigg|_{-\infty}^{+\infty} 
- \int \frac{-\sigt}{\sigs}\phi(\varepsilon)\phi\left(z^*\right) \dd \varepsilon \\
=&\frac{\sigt}{\sigs}\int\phi\left(z^*\right) \dd \Phi(\varepsilon)
\end{align*}
and
\begin{align*}
\int\frac{\sigs}{(1+\gamma)^2}{\gamma'}_\theta \phi\left(z^*\right) \dd \Phi(\varepsilon)
= \int \frac{-2(\sigs/\sigt)\gamma}{(1+\gamma)^2 }\phi\left(z^*\right) \dd \Phi(\varepsilon).
\end{align*}
Therefore, (\ref{eq:Dt1}) becomes
$$\frac{(1+3\gamma)(\sigt/\sigs) +2(\sigs/\sigt)\gamma }{(1+\gamma)^2}
\int \phi\left(z^*\right) \dd \Phi(\varepsilon)>0.$$
Hence $D(\cdot)$ increases in $\sigt$.

Lastly, we show $D(\cdot)$ decreases in $\sigs$.
Denote
$${\gamma'}_s= \frac{\partial \gamma}{\partial \sigs} 
= \frac{2\sigs}{\sigt^2}$$
and 
$${z'}_s= \frac{\partial z^*}{\partial \sigs} 
= \frac{(\overline{v}-x){\gamma'}_s - \sigs z^*}{\sigma_s^2}.$$
Taking partial derivative of (\ref{eq:D1}) with respect to $\sigs$, we can find
$$(\overline{v}-x)\int {z'}_s \phi\left(z^*\right) \dd \Phi(\varepsilon).$$
Taking partial derivative of (\ref{eq:D2a}) with respect to $\sigs$, we can find
\begin{align*}
&-\int\frac{-\sigt\varepsilon{\gamma'}_s}{(1+\gamma)^2}\Phi\left(z^*\right)
+\frac{\sigt\varepsilon}{1+\gamma}{z'}_s \phi\left(z^*\right) \dd \Phi(\varepsilon).
\end{align*}
Taking partial derivative of (\ref{eq:D3}) with respect to $\sigs$, we can find
$$-\int \frac{(1+\gamma)-\sigs{\gamma'}_s}{(1+\gamma)^2}\phi\left(z^*\right) 
+ \frac{\sigs}{1+\gamma}{z'}_s (-z^*)\phi\left(z^*\right) \dd \Phi(\varepsilon).$$
Summing up, the partial derivative becomes
\begin{align}
&\int\frac{\sigt\varepsilon{\gamma'}_s}{(1+\gamma)^2}\Phi\left(z^*\right)\dd \Phi(\varepsilon)
-\int \frac{(1+\gamma)-\sigs{\gamma'}_s}{(1+\gamma)^2}\phi\left(z^*\right) \dd \Phi(\varepsilon)\nonumber\\
=&-\frac{\sigt{\gamma'}_s}{(1+\gamma)^2}\frac{\sigt}{\sigs}\int \phi\left(z^*\right) \dd \Phi(\varepsilon)
-\frac{(1+\gamma)+2\gamma}{(1+\gamma)^2}\int \phi\left(z^*\right) \dd \Phi(\varepsilon)\nonumber\\
=&\frac{-3}{1+\gamma}\int \phi\left(z^*\right) \dd \Phi(\varepsilon)<0.
\end{align}
Hence $D(\cdot)$ decreases in $\sigs$,
which implies $D(\cdot)$ decreases in $\gamma\equiv\frac{\sigs^2}{\sigt^2}$.

It is trivial that $D(\cdot)$ decreases in $c$.

==> old_result.tex <==

Figure \ref{fig:errors} shows the average belief errors in efficacy and hospitalization prevention rates under each information demand category.
On average, the Top 3 vaccines have lower pre-treatment errors,
which indicates that the subjects tend to consume the information that they have already had some knowledge about.%\footnote{See discussions in Section ??.} 
From the figure, we can also see that the drops in error after receiving the information are the largest in the Not Top 3 group. 
This implies that the subjects may learn more from the information if the information did not interest the subjects. 

Figure \ref{fig:errors_scatter} gives a similar observation with scatter plots.
The fitted lines are based on the linear specifications regressing post-treatment error on the pre-treatment error,
where the 45-degree line means no updates at all (the errors are not reduced after receiving information),
and the 0-degree line means full update.
Among the three categories, the fitted lines of the Not Top 3 vaccines distort toward the 0-degree line the most (comparing the received and the not received),
which suggests that the subjects adjusted their beliefs toward the information more for the Not Top 3 vaccines.
The OLS estimation supports the observations found in the graphs.
The slope change in the Not Top 3 vaccines is -0.16 (standard error 0.06) for efficacy and -0.19 (standard error 0.06) for hospitalization prevention rate. 
The slope change in the Selected Top 3 and Not Selected Top 3 are not significantly different from 0 for either efficacy or hospitalization prevention rate (see Table \ref{tab:error_group}).
We will elaborate more about the learning in Section \ref{sec:learning}.

\begin{result}
On average, the subjects select the information they have smaller errors about.
However, the subjects adjust their beliefs more when they receive the Not Top 3 vaccine information.
\end{result}

\begin{figure}
{
\centering
\includegraphics[width=0.48\linewidth]{group_bar_efficacy_error.png}
\includegraphics[width=0.48\linewidth]{group_bar_efficacy_rest.png}\\

\includegraphics[width=0.48\linewidth]{group_bar_hospital_error.png}
\includegraphics[width=0.48\linewidth]{group_bar_hospital_rest.png}
\caption{The mean errors before and after the treatments}
\label{fig:errors}
}
\begin{minipage}{\linewidth}
\footnotesize
\emph{Note:} Each bar represents the mean error in each category.
Within each category, the left/lighter one is for the observations that the subjects do not receive the vaccine information,
and the right/deeper one is for the observations that the subjects receive the information.
95\% confidence intervals of the means are plotted for each category.
\end{minipage}
\end{figure}



\begin{figure}
{
\centering
\includegraphics[width=0.48\linewidth]{group_scatter_efficacy_error.png}
\includegraphics[width=0.48\linewidth]{group_scatter_hospital_error.png}
\caption{The distribution of errors before and after the treatments}
\label{fig:errors_scatter}
}
\begin{minipage}{\linewidth}
\footnotesize
\emph{Note:} Each bin contains around 50 observations.
The median is plotted within each bin.
The dashed red lines are the 45-degree line and the 0-degree line.
Each of the solid lines is the OLS fitted line for each of the categories.
The hollow dots and the lighter lines represents the observations that the subjects do not receive any information.
\end{minipage}


\end{figure}



\subsection{Learning from the Information}
	\label{sec:learning}
One way to measure the learning from the information is to see 
how much the pre-treatment errors are reduced after the subjects acquired the information.
We may define learning as the difference between the pre-treatment and post-treatment errors,
$$\text{Learning}_{i,v} = |\text{Error}^{Pre}_{i,v}| - |\text{Error}^{Post}_{i,v}|.$$
That is, the larger the learning is, the more the error is reduced.
Table \ref{tab:summary_main} also summarizes statistics for learning. 
On average, the learning is 0.70 (standard deviation 14.85) in efficacy and 4.01 (standard deviation 21.26) in hospitalization prevention rate.

Figure \ref{fig:learning_in_beliefs} depicts the learning under each information demand category.
We first focus on the treatment effects within each category.
For the top-3-ranked vaccines, the difference in learning between the received and not received is not significant, while the difference in learning is significantly different for the vaccines that are not in the subjects' top 3.

We can further estimate the following regression model to see the heterogeneity in learning among different information demand categories:
$$ \text{Learning}_{i,v} = \alpha + \sum_{k\in \mathcal{D}}\delta_k D^k_{i,v} + X'_{i}\xi + \varepsilon_{i,v}, $$
where  $D^k_{i,v}$ are the category variables indicating which category (according to subject $i$'s demand and the reception of the information) vaccine $v$ belongs to, and $\mathcal{D}$ contains all categories except the not-received Not Top 3 vaccines.
Table \ref{tab:learning} quantitatively shows the estimates on learning, which suggests a similar finding from the figures.
The bottom rows are the differences between the received and non-received within each demand group.
For efficacy, the difference in Not Top 3 vaccines is 4.50 (out of 100, standard error 1.06), 
1.36 (standard error 0.75) in Selected Top 3,
and 1.15 (standard error 1.54) in Not Selected Top 3.
For the hospitalization prevention rate, the difference in Not Top 3 vaccines is 6.34 (standard error 1.50), 
0.56 (standard error 1.34) in Selected Top 3,
and -0.43 (standard error 2.13) in Not Selected Top 3.
The learning in Not Top 3 vaccines is quantitatively higher than in the Top 3 vaccines.
The Wald tests comparing the learning effects between the Not Top 3 and the Top 3 also suggest a significant difference.
In models (3) and (4), we include the pre-treatment errors to control the first-order effects from the misbelief prior to the information treatment,
and the above findings remain robust. 

\begin{figure}
{\centering
%	\begin{subfigure}[t]{\textwidth}
%	\centering
	\includegraphics[width=0.45\textwidth]{group_bar_efficacy_learning.png}
	\includegraphics[width=0.45\textwidth]{group_bar_hospital_learning.png}
%	\caption{learning}
%	\label{fig:learning_raw_in_beliefs}
%	\end{subfigure}
%	
%	\begin{subfigure}[t]{\textwidth}
%	\centering
%	\includegraphics[width=0.45\textwidth]{group_bar_efficacy_lratio.png}
%	\includegraphics[width=0.45\textwidth]{group_bar_hospital_lratio.png}
%	\caption{learning per pre-treatment error}
%	\label{fig:lratio_in_beliefs}
%	\end{subfigure}
	\caption{Learning in Beliefs}
	\label{fig:learning_in_beliefs}
}
\begin{minipage}{\linewidth}
\footnotesize
\emph{Note:} Each bar represents the mean learning (reduction in errors before and after the information exposure stage) in each category.
Within each category, the left/lighter one is for the observations that the subjects do not receive the vaccine information,
and the right/deeper one is for the observations that the subjects receive the information.
95\% confidence intervals of the means are plotted for each category.
\end{minipage}
\end{figure}

\begin{table}[htp]
\centering
\caption{Learning}\label{tab:learning}
{ \small 
\input{tables/learning_group.tex}
}
\end{table}

We also look at the observations with the pre-treatment errors in beliefs below the median to control the pre-treatment misbelief.
Table \ref{tab:learning_belowmed} shows the results.
We find not only that the treatment effect in the Not Top 3 vaccines vanishes,
but the effect in Selected Top 3 vaccines becomes significantly different from zero.
The results suggest that the learning in Not Top 3 vaccines comes mostly from the vaccines that the subjects knew less about.

\begin{result}
The learning from the information is the largest in the Non Top 3 category.
However, if we focus on the observations with lower pre-treatment errors,
the learning in the Selected Top 3 category becomes the most prominent.
\end{result}

\begin{table}[htp]
\centering
\caption{Learning (Below Median)}\label{tab:learning_belowmed}

{ \small 
\input{tables/learning_group_belowmed.tex}
}


\end{table}



==> preference_reg_full.tex <==
\\ \hline\hline
&
\multicolumn{2}{c}{
PostPreference
$-$
PrePreference
}\\
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         \\
\hline
                    &                     &                     \\
\emph{Belief Differences}&                     &                     \\
Efficacy            &        0.08\sym{**} &       -0.00         \\
                    &      (0.03)         &      (0.04)         \\
Hospitalization     &        0.11\sym{***}&        0.10\sym{*}  \\
                    &      (0.02)         &      (0.04)         \\
Adverse Events      &       -0.05\sym{**} &       -0.05         \\
                    &      (0.02)         &      (0.03)         \\
Severe Adverse Events&       -0.03         &       -0.02         \\
                    &      (0.02)         &      (0.04)         \\
\emph{Information Demand}&                     &                     \\
Selected Top 3 -- Received&        1.41         &        1.39         \\
                    &      (0.80)         &      (0.89)         \\
\qquad \dots $ \times $  Efficacy&                     &        0.11         \\
                    &                     &      (0.06)         \\
\qquad \dots $ \times $  Hospitalization&                     &       -0.01         \\
                    &                     &      (0.04)         \\
\qquad \dots $ \times $  Adverse Event&                     &        0.02         \\
                    &                     &      (0.03)         \\
\qquad \dots $ \times $  Severe AE&                     &       -0.03         \\
                    &                     &      (0.04)         \\
-- Not Received     &       -1.35         &       -2.64         \\
                    &      (1.22)         &      (1.58)         \\
\qquad \dots $ \times $  Efficacy&                     &        0.26\sym{**} \\
                    &                     &      (0.09)         \\
\qquad \dots $ \times $  Hospitalization&                     &       -0.01         \\
                    &                     &      (0.06)         \\
\qquad \dots $ \times $  Adverse Event&                     &       -0.01         \\
                    &                     &      (0.04)         \\
\qquad \dots $ \times $  Severe AE&                     &       -0.06         \\
                    &                     &      (0.06)         \\
Not Selected Top 3 -- Received&       -1.64         &       -2.30         \\
                    &      (1.61)         &      (1.95)         \\
\qquad \dots $ \times $  Efficacy&                     &        0.22\sym{*}  \\
                    &                     &      (0.09)         \\
\qquad \dots $ \times $  Hospitalization&                     &       -0.04         \\
                    &                     &      (0.06)         \\
\qquad \dots $ \times $  Adverse Event&                     &       -0.06         \\
                    &                     &      (0.06)         \\
\qquad \dots $ \times $  Severe AE&                     &        0.05         \\
                    &                     &      (0.08)         \\
 -- Not Received    &        0.33         &        0.02         \\
                    &      (1.29)         &      (1.45)         \\
\qquad \dots $ \times $  Efficacy&                     &        0.00         \\
                    &                     &      (0.11)         \\
\qquad \dots $ \times $  Hospitalization&                     &        0.04         \\
                    &                     &      (0.07)         \\
\qquad \dots $ \times $  Adverse Event&                     &       -0.05         \\
                    &                     &      (0.07)         \\
\qquad \dots $ \times $  Severe AE&                     &       -0.04         \\
                    &                     &      (0.07)         \\
Not Top 3 -- Received&       -1.16         &       -1.81         \\
                    &      (1.34)         &      (1.58)         \\
\qquad \dots $ \times $  Efficacy&                     &        0.12         \\
                    &                     &      (0.07)         \\
\qquad \dots $ \times $  Hospitalization&                     &        0.07         \\
                    &                     &      (0.06)         \\
\qquad \dots $ \times $  Adverse Event&                     &       -0.03         \\
                    &                     &      (0.05)         \\
\qquad \dots $ \times $  Severe AE&                     &        0.06         \\
                    &                     &      (0.06)         \\
Constants           &        1.63         &        1.82         \\
                    &      (2.07)         &      (2.05)         \\
\hline
Treatment Effects in \dots&                     &                     \\
Selected Top 3      &        2.77\sym{**} &        4.02\sym{**} \\
                    &      (1.02)         &      (1.44)         \\
Not Selected Top 3  &       -1.97         &       -2.32         \\
                    &      (1.91)         &      (2.41)         \\
Not Top 3           &       -1.16         &       -1.81         \\
                    &      (1.34)         &      (1.58)         \\
\hline
Observations        &        3160         &        3160         \\
Subjects            &         632         &         632         \\
 $ R^2 $            &       0.052         &       0.062         \\
Mean of Dep. Variable&       0.035         &       0.035         \\
 \hline\hline \\
\multicolumn{3}{l}{
\begin{minipage}{0.5\textwidth}
Standard errors in parentheses.  The subjects' family income, college majors, and sex are controlled. \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)
\end{minipage}
}


==> remarks.tex <==
\section{Remarks}
\subsection{Demands in Vaccine Information}
What vaccine information does our subjects want to know the most?

\subsection{The Reception of the Information}
In the analysis, the reception is defined by whether the information is delivered to the subjects.
However, it is possible that the subjects did not pay attention to the information.
To investigate the information reception more closely,
we collect the mouse click behavior on each attributes of the vaccine information.
On the information page, the subjects have to click on the button to see the information, 
as shown in Figure \ref{info_sheet}.


\subsection{The Spill-over Effects of the Information}
It is also possible that the subjects might still update their beliefs about the uninformed vaccines.



==> summary_errors.tex <==
                    &    Efficacy&Hospitalization&Adverse Event&   Severe AE\\
\hline
Pre-treatment Belief $-$ Information &       12.98&       25.40&       -15.46&       -32.02\\
                    &     (22.45)&     (25.05)&     (35.85)&     (29.34)\\
[1em]
$|$ Pre-treatment Belief $-$ Information $|$&       18.61&       26.25&       32.27&       32.07\\
                    &     (18.05)&     (24.16)&     (21.98)&     (29.28)\\
[1em]
Post-treatment Error &       9.88&       20.62&       -7.30&       -28.42\\
                    &     (24.09)&     (26.26)&     (37.19)&     (28.42)\\
[1em]
$|$ Post-treatment Error $|$&       17.92&       22.23&       30.62&       28.50\\
                    &     (18.89)&     (24.90)&     (22.32)&     (30.34)\\
%[1em]
%Learning            &       0.696&       4.011&       1.645&       3.570\\
%                    &     (14.85)&     (21.26)&     (23.45)&     (24.15)\\


==> update.tex <==
\begin{tabular}{l*{6}c}\hline\hline
&
\multicolumn{6}{c}{\emph{Belief
Update}:
}\\
&
\multicolumn{6}{c}{Post-Treatment
Belief
$-$
Pre-Treatment
Belief
}\\
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
                    &    \multicolumn{3}{c}{Efficacy}        & \multicolumn{3}{c}{Hospitalization} \\
\hline
Selected Top 3      &        2.82\sym{*}  &        2.83\sym{*}  &        5.77\sym{***}&        4.40\sym{**} &        4.36\sym{**} &        1.95         \\
                    &      (1.15)         &      (1.16)         &      (1.09)         &      (1.42)         &      (1.43)         &      (1.53)         \\
Not Selected Top 3  &        0.06         &       -0.23         &       -0.85         &        0.75         &        0.59         &        0.53         \\
                    &      (1.43)         &      (1.44)         &      (2.30)         &      (1.73)         &      (1.76)         &      (2.41)         \\
Signal Strength     &        0.28\sym{***}&        0.26\sym{***}&                     &        0.63\sym{***}&        0.58\sym{***}&                     \\
                    &      (0.04)         &      (0.03)         &                     &      (0.05)         &      (0.05)         &                     \\
Signal Strength of Other Vaccines&                     &        0.05         &        0.13\sym{**} &                     &        0.05         &        0.37\sym{***}\\
                    &                     &      (0.04)         &      (0.04)         &                     &      (0.04)         &      (0.04)         \\
Constants           &       -1.55         &       -1.77         &       -2.95         &      -10.91\sym{**} &      -11.14\sym{**} &       -9.59\sym{**} \\
                    &      (2.13)         &      (2.11)         &      (2.87)         &      (3.44)         &      (3.51)         &      (3.69)         \\
\hline
Observations        &        1762         &        1741         &        1209         &        1762         &        1741         &        1209         \\
Subjects            &         611         &         590         &         590         &         611         &         590         &         590         \\
 $ R^2 $            &        0.20         &        0.20         &        0.11         &        0.34         &        0.34         &        0.21         \\
Mean of Dep. Variable&        4.26         &        4.24         &        1.15         &        6.65         &        6.63         &        2.35         \\
Info Received?      &         Yes         &         Yes         &          No         &         Yes         &         Yes         &          No         \\
 \hline\hline \end{tabular}\\ \begin{tfootnote}                 Clustered (on subject level) standard errors in parentheses. Pre-Treatment beliefs, the subjects' family income, college majors, and sex are controlled.                  The signal strength of other vaccines is the average of the signal strength from other vaccines.                 When there is no other information received, the observation will be dropped in models (2), (3), (5), and (6).                 \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\) . \end{tfootnote}

